Automated Contrastive Learning Strategy Search for Time Series

In recent years, Contrastive Learning (CL) has become a predominant representation learning paradigm for time series. Most existing methods manually build specific CL Strategies (CLS) by human heuristics for certain datasets and tasks. However, manually developing CLS usually requires excessive prior knowledge about the data, and massive experiments to determine the detailed CL configurations. In this paper, we present an Automated Machine Learning (AutoML) practice at Microsoft, which automatically learns CLS for time series datasets and tasks, namely Automated Contrastive Learning (AutoCL). We first construct a principled search space of size over $3\times10^{12}$, covering data augmentation, embedding transformation, contrastive pair construction, and contrastive losses. Further, we introduce an efficient reinforcement learning algorithm, which optimizes CLS from the performance on the validation tasks, to obtain effective CLS within the space. Experimental results on various real-world datasets demonstrate that AutoCL could automatically find the suitable CLS for the given dataset and task. From the candidate CLS found by AutoCL on several public datasets/tasks, we compose a transferable Generally Good Strategy (GGS), which has a strong performance for other datasets. We also provide empirical analysis as a guide for the future design of CLS.

==> 02_preliminary.tex <==
\section{Preliminary}


\begin{definition}[Contrastive Strategy Search for Time Series]
Denote $\mathcal{D}$ and $\mathcal{T}$ as the time series dataset and the downstream task.
Let $\mathcal{S}$ be the search space comprised of various choices of contrastive strategies.
The task is to build a function $f$ to automatically find a the optimal strategy $s\in\mathcal{S}$. 
\end{definition}

==> 05_related_work.tex <==
\section{Related Work}
% In this section, we briefly review time series contrastive learning methods and automated contrastive learning methods.
% \kan{we may need to mention non-contrastive self-supervised learning on time series. we can point out that: Because of the generality of our automation methodology, we believe that our proposed framework could be transferred to non-contrastive self-supervised learning on time series, which we leave as our future work.}

\textbf{Time Series Contrastive Learning.}
Contrastive learning aims to train encoders that can learn informative embeddings by distinguishing positive data pairs and negative data pairs \cite{liu2021self}, and it has been demonstrated to be effective in domains such as computer vision \cite{ozbulak2023know}, natural language processing \cite{zhang-etal-2022-contrastive-data} and graph mining \cite{liu2022graph}.
In recent years, some studies introduce contrasive learning into the time series domain and have achieved impressive performance \cite{zhang2023self}.
SRL \cite{franceschi2019unsupervised} proposes to treat two adjacent sub-sequences from the same time series as positive pairs, and sub-sequences from other time series as negative samples.
CPC \cite{oord2018representation} introduces the popular InfoNCE loss.
Self-EEG \cite{sarkar2020self} augments the input EEG signals with various transformations. 
TNC \cite{tonekaboni2020unsupervised} constructs contrastive pairs based on the local smoothness of time series.
TS-TCC \cite{eldeletime} transforms the input data with weak and strong augmentations, and use temporal and contextual contrasting to train the encoders.
Instead of only considering data augmentations in the temporal domain, CoST \cite{woo2021cost}, BTSF \cite{yang2022unsupervised} and TF-C \cite{zhang2022self} further propose to augment time series in the frequency domain.
TS2Vec \cite{yue2022ts2vec} obtains time series representations of multiple scales by hierarchical pooling and performs CL at each scale.
% Despite the great performance achieved by these methods, they are ad-hoc for different datasets and tasks.
% TimesURL \cite{liu2023timesurl} augments a time series data point (or embedding) by injecting data (embedding) from other time series as noise.
To reduce human efforts in finding the optimal data augmentations, InfoTS \cite{luo2023time} recently proposes to automatically select data augmentations through meta-learning.
However, InfoTS only considers data augmentations yet ignores other critical components in contrastive learning such as embedding transformation, contrasive pair construction and loss functions.
Besides, InfoTS selects data augmentations based on a dataset/task-agnostic criteria, which is less effective in capturing the characteristics of the datasets and downstream tasks and thus might not be able find the optimal solution.
Compared with InfoTS, \autocss\ 
(1) considers a larger search space comprised of data augmentations, emebedding transformations, and loss functions;
(2) finds the optimal strategy based on the model's performance on the validation set.

\textbf{Automated Contrastive Learning.}
Despite various powerful contrastive strategies have been developed for particular datasets and downstream tasks, 
they cannot be easily adapted to other datasets and tasks \cite{luo2023time,tian2020makes,you2021graph}.
Therefore, it is necessary to develop automatic searching algorithms to find the optimal contrastive strategies for a given dataset and task.
In the computer vision domain, 
InfoMin \cite{tian2020makes} introduces a mutual information minimization criteria for selecting augmented views.
SelfAugment \cite{reed2021selfaugment} uses the self-supervised image rotation task to guide the selection of data augmentations.
In the graph domain,
JOAO \cite{you2021graph} presents a Bayesian framework to adaptively find the optimal data augmentations.
AutoSSL \cite{jin2021automated} learns the weights of different contrastive strategies.
AutoGCL \cite{yin2022autogcl} builds an end-to-end framework to automatically learn the distributions of node level augmentations.
In the time series domain, InfoTS \cite{luo2023time} recently propose to adaptively select the optimal data augmentations based on information theory.
Different from previous studies which mainly focus on searching the optimal data augmentations, in this paper, we propose \autocss\ to simultaneously consider various dimensions of CL, including data augmentations, embedding transformations, contrastive pair construction and loss functions.

